1-Lipschitz Layers Compared: Memory, Speed, and Certifiable Robustness

The robustness of neural networks against input perturbations with bounded magnitude represents a serious concern in the deployment of deep learning models in safety-critical systems. Recently, the scientific community has focused on enhancing certifiable robustness guarantees by crafting 1-Lipschitz neural networks that leverage Lipschitz bounded dense and convolutional layers. Although different methods have been proposed in the literature to achieve this goal, understanding the performance of such methods is not straightforward, since different metrics can be relevant (e.g., training time, memory usage, accuracy, certifiable robustness) for different applications. For this reason, this work provides a thorough theoretical and empirical comparison between methods by evaluating them in terms of memory usage, speed, and certifiable robust accuracy. The paper also provides some guidelines and recommendations to support the user in selecting the methods that work best depending on the available resources. We provide code at https://github.com/berndprach/1LipschitzLayersCompared.

==> fig/train_memory.tex <==


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{pics/TrainingMemoryRequirements.png}
    \caption{\bp{Not yet evaluated on A100!} Training memory requirements 
    of different layers for different model sizes.}
    \label{fig:trainingmemory}
\end{figure}





==> fig/train_val_times.tex <==


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{pics/time_and_memory/training_time_per_epoch.pdf}
    \includegraphics[width=\columnwidth]{pics/time_and_memory/forward_throughput.pdf}
    \caption{
        \textbf{Training time} per epoch (on \CIFARS) 
        as well as 
        \textbf{\Inference throughput} (examples per second)
        for different layers types and different model size.
        Assumes all parameter transformations
        have been evaluated and cached beforehand.
        \bp{\SLL did not have caching yet!}
    }
    \label{fig:trainingtimes}
\end{figure}


==> fig/val_memory.tex <==



\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{pics/ForwardPassMemoryRequirements.png}
    \caption{\bp{Not yet evaluated on A100!} Memory requirements
    in order to do a forward pass for one batch of inputs.}
    \label{fig:validationmemory}
\end{figure}






==> sec/3_summary.tex <==
\section{Lipschitz Bounded layers \bp{OLD version}}
In this section we summarize methods from the literature \bp{in chronological order?}, 
with some added observations from our side? \bp{Correct?}
\subsection{Notation and Background}
Henceforth we refer to $\OO(n)$ as the space of square orthogonal matrices of size $n$ and to $\PP(m,n)\subseteq\R^{m\times n}$ as the set of all the symmetric projections, i.e.$P^2=PP^T=I$. We consider a kernel $W$ as a 4-dimensional tensor of $\R^{c \times d \times k_1 \times k_2}$ where $c, d, k$ are respectively the \textit{output dimension}, \textit{input dimension} and \textit{kernel size} or \textit{filter dimension}. We say that a layer $f:\R^m\to\R^n$ is orthogonal if the corresponding Jacobian matrix in $0$ is orthogonal. A kernel $W$ is said to be orthogonal if the inducted convolution with circular padding is an orthogonal layer, and $\OO(c,k)$ represents the space of all the orthogonal kernels with a filter size of $k$. Observe that, since convolution with zero padding and filter size greater than $1$ can not be orthogonal, see \cite[App.D.2]{bcop}, we only refers to convolutions with circular padding for the orthogonal convolutional layers. Zero padding is still considered for those methods that provide 1-Lipschitz convolutional layers.

\paragraph{Spectral Normalization}
Spectral normalization strategy has been first presented in \cite{miyato} and provides 1-Lipschitz fully connected and convolutional layer. The strategy relies on the power method in order to obtain an estimation \textemdash of a lower bound \textemdash of the spectral norm of the weight matrix. Despite for the fully connected case the power method is directly applied to the weight matrix, for the convolutional case instead the power method is applied to a reshaped version of the 4-dimensional weight $W$. In detail, if $W\in\R^{c\times d\times h \times w}$ represents the kernel of the convolution, the spectral norm of the convolutional operator $x \mapsto W \star x$ is deduced by estimating the spectral norm of the matrix $\hat W\in\R^{c\times dhw}$ and rescaling it by some constant factor $K$ that depends on the filter size. 

The exact value of the constant $K$ is not provided by \cite{miyato}, but can be deduced from \cite{fantastic4} to be $K=\sqrt{hw}$ since the reshaped matrix $\hat W$ concides to the matrix $T$.

A tight bound of the spectral norm is proposed in \cite{fantastic4} in which the authors adapt the proof of the exact estimation of the singular values of convolutional layers in \cite{Sedghi_2019} to provide an upper-bound of the largest singular value of the convolutional operator. Such a upper bound is differentiable and can be directly used to rescale the convolutional kernel in order to obtain a 1-Lipschitz convolution \todo{Complet Fantastic of Singla}

\bp{Should we have a subsection "General Tool" or so for BnB and PI?}
\paragraph{Bjorck \& Bowie}
Bjorck \& Bowie \cite{Bjorck_1971_SIAM} introduced an iterative algorithm that find the closest orthogonal matrix to an input matrix.
The algorithm is furthermore differentiable, which makes it a very useful tool for many \ols-layers
that rely on orthogonal matrices.
The algorithm can also directly be used to create orthogonal layers.
It was used for example by \cite{anil_fc} in order to construct a \ols network.
We use it (with the same number of iterations) to directly to parameterize 
$1 \times 1$ convolutions and fully connected layers.

\cite{anil_fc}
\begin{obs}[Algorithimic Complexity]
Given a matrix $A\in \Ch^{c\times d}$, let $A_k$ defined as follows
\begin{equation}
    A_{k+1} = A_k\left(I + \frac12 Q_k \right),\quad\mbox{where}\quad Q_k=I-A_k^HA_k
\end{equation}
where $A_0=A$.
The computational cost of $A_k v$ can be deduced iteratively by considering
\begin{equation}
    A_{k+1} v = A_k\left(\frac32 I - \frac12 A_k^HA_k\right)v
    = \frac32 \underbrace{A_k v}_{O(cd)} - \underbrace{A_kA_k^HA_k v}_{3O(cd)}
\end{equation}
hence the computational cost of the algorithm with $t$ iterations is $4t O(mn)$. Empirical evaluations show that $t=20$ is sufficient to reach the convergence.
\end{obs}
\cite{anil_fc}

(\BCOP reduces to \BnB for $1\times1$ convolutions.)


\paragraph{Power Method}
The \emph{Power Method} was used in \cite{Miyato_2018_ICLR} and \cite{CPL} in order to bound the
spectral norm of matrices. It starts with a random initialized vector $\vec{u}$,
and iteratively applies the following:
\begin{equation}
    \vec{v} = \frac{W^\top \vec{u}}{\|W^\top \vec{u}\|_2}, \quad
    \vec{u} = \frac{W \vec{v}}{\|W \vec{v}\|_2}.
\end{equation}
Then we can approximate the spectral norm of $W$ as
\begin{equation}
    \spect{W} \sim \vec{u}^\top W \vec{v}.
\end{equation}
Notably, since the weight matrices usually change only slightly at each training
step, we can store and reuse the vector $\vec{u}$ in each forward pass.
This allows us to only do one iteration at each training step,
and makes the power method cheap to apply during training.

We can also efficiently use the \powermeth for convolutional layers.
This was done for example already by \cite{Farnia_2018_ICLR,GloRo}.
% by relying on a transposed convolution (instead of transposing the Jacobian itself)
% For this,by relying on a transposed convolution (instead of transposing the Jacobian itself)
In particular, we can transpose (and flip) the convolution kernel in a certain way
in order to obtain a (transposed) convolution with its Jacobian being the transpose
of the Jacobian of the original layer.

The \powermeth is usually not differentiated through.

We have tried using the power method by itself to construct
a \ols layer, however in preliminary experiments the performance
was quite poor compared to other methods, so we do not report
results for it. \bp{?}
\textbf{We furthermore found that 100 iterations 
(which are used by papers such as \cite{GloRo}) are often not enough to
estimate the Lipschitz constant of the network accurately enough,
casting doubt on their reported results.}
We use the \emph{Power Method} in order to (double) check the
Lipschitz constant of other iterative methods such as \SOC.
For this we choose to do 10.000 iterations.

\paragraph{BCOP}
The \textit{Block Orthogonal Convolution Parameterization} is introduced in \cite{bcop} by extending the work of \cite{dynamical_isometry} in which explicitly orthogonal kernels are provided. The base idea of the two works relies on the construction of orthogonal convolutions whose kernels $W\in\R^{c \times c \times k \times k}$ are written as a \textit{Block Convolutional Product} and combination of $k$ orthogonal matrices. 
The block convolutional product can be though as a convolution between tensors where the element wise product is replaced by a matrix product.

\begin{defn}[Block Convolution]
Let $X\in\R^{m\times n \times h_1\times h_2}$ and let $X_{ij}\in\R^{m\times n}$ for each $i,j$. Given a second kernel $Y\in\R^{n\times d \times w_1\times w_2}$ we define $X\square Y\in\R^{m\times d\times k_1\times k_2}$ as 
\begin{equation}
\left(X\square Y\right)_{ij} = \sum_{\mu,\nu=-\infty}^\infty
X_{\mu\nu}Y_{i-\mu,j-\nu}
\end{equation}
where the $X_{\mu\nu}$ and $Y_{\mu\nu}$ are assumed zeros for out-of-range index, and $k=h+w-1$.
\end{defn}
Under this definition, an orthogonal kernel $W=W(H,P_{1:k},Q_{1:k})$ can be explicitly represented as follows
\begin{equation}
    W = H\square W_1 \square\cdots\square W_{k-1}
\end{equation}
where $H\in\R^{c\times c\times 1\times 1}$ is an orthogonal kernel with filters of dimension $1$, and $W_i$
are obtained by 
\begin{equation}
\R^{c\times c\times 2\times 2}\ni
    W_i =
    \begin{bmatrix}
    I & (I-P_i)
    \end{bmatrix}
    \square
    \begin{bmatrix}
    I\\
    I - Q_i
    \end{bmatrix},
\end{equation} where $P_i,Q_i\in\R^{c\times c}$ are symmetric projection matrices, i.e. $P^2=PP^T=I$.

Such a orthogonal parameterized kernels $W(H,P_{1:k},Q_{1:k})$ constitute a sub-manifold of all the possible orthogonal kernels
\begin{equation}
    \WW(c,k):=\left\{
    W(H,P_{1:k},Q_{1:k})\,|\, H\in\OO(c)\,, P_i,Q_i\in\PP(c)
    \right\} \subset \OO(c,k).
\end{equation}
However, since $\WW(c,2)$ has at least $2(c+1)^2$ connected components, \cite[Thm.2]{bcop}, optimizing over such a parametric orthogonal kernel can be a tough problem. Indeed, the parameter of models optimized through gradient-base optimization strategies could be confined to remain in its initial connected component. 
To overcame this issue, authors showed that any kernel
$W=W(H,P_{1:k},Q_{1:k})$ can be represented as a projection on the first $n$ channels of a kernel $\tilde W\in\WW(2n,k)$ obtained by $\tilde W = W(\tilde H, \tilde P_{i:k}, \tilde Q_{1:k})$ where $\tilde P_i,\tilde Q_i\in\PP(2c,c)$. Furthermore, kernels $\tilde W$ all live in the same connected component. 
In conclusion, authors leverage Bjorck and Bowie algorithm for crafting the orthogonal matrix $H$ and the projection matrices $P_i, Q_i$ (obtained by considering $Q = (A^TA)^{-\frac12}$, see \cite{Bjorck_1971_SIAM} for further details.).
\newline

\noindent
\textbf{Remark.} As a result of this procedure, BCOP parameterizes an orthogonal kernel in $\OO(n,k)$ by leveraging an orthogonal matrix $H\in\R^{c\times c}$ and $k-1$ $\left\lfloor\frac{c}{2}\right\rfloor$-rank couples of projections, resulting in $c^2 + 2(k-1)c\left\lfloor\frac{c}{2}\right\rfloor = kc^2$ parameters, less than the $k^2c^2$ parameters of a plain convolution. \todo{BCOP: Not clear. infer these numbers from the code}



\paragraph{Cayley}
\cite{caley}
\todo{Description Cayley}


\paragraph{SOC}
\cite{soc}
\todo{Description SOC}


\paragraph{AOL}
The \emph{Almost Orthogonal Lipschitz} layers where introduced in \cite{aol}.
The method computes an upper bound of the spectral norm of matrices.
This bound is used to rescale the inputs of a layer in a way that makes the full operation \ols.
The bound is tight for orthogonal matrices, and can be extended efficiently to convolutions.


\paragraph{LOT}
\cite{lot}


\paragraph{CPL}
In \cite{CPL} the authors proposed the \emph{Convex Potential Layer}.
For $\sigma$ a non-decreasing \ols function (usually ReLU), it is given as
\begin{equation}
    l(x) = x - \frac{2}{\|W\|_2^2} W^\top \sigma(Wx + b).
\end{equation}
The spectral norm is approximated using Power Iteration.

\paragraph{SLL}
\emph{SDP-based Lipschitz Layers (SLL)} \cite{SLL} combine 
the \CPL layer
with the upper bound on the spectral norm from AOL.

Both \CPL as well as \SLL are not-linear by construction, so they can be
used to construct a network without any further use of activation functions.
However, we've found \bp{Checking that atm!} that alternating \SLL layers
and \MaxMin activations seems to work better empirically.

==> sec/4_comparison_OLD.tex <==

\section{Theoretical Comparisons}

For an overview of results see \cref{table:theoretical}
% \input{tab/theoretical_both}

As evident in the last section there
are various ideas and methods on how to 
parameterize \ols convolutions.
These causes the different methods to have very different
properties and requirements.
In this section we try to (theoretically)
summaries the 
properties (especially algorithmic complexity)
of different algorithms,
and provide a comparison of them.

% \paragraph{Analysis of the Memory Usage (?)}
% To Be discussed since strongly depends on the implementation
\fb{Summury of the aim of the section and referemnts to link and tables}

\paragraph{Analysis of the Algorithmic Complexity}
% Computational cost depending on the input features and/or channels and/or feature map dimension
It is a very important property on neural networks
how fast we can evaluate the output of the model
at training time,
so we can train the model in reasonable time
and for a lot of epochs.
Maybe it is even more important how quickly 
we can evaluate the model output at test time, 
since this determines how useful 
(and maybe also how expensive)
the model would be in production.

Furthermore, we also often do want scale either the input size
or the number of parameters of our models.
%
In order to give an overview on how these scaling
effect the time requirements for different methods
of creating \ols networks, we have summarized
their computational complexity in \cref{table:complexity}.
In the column \textit{Training}, the leading terms of the computation can be found. 
For the sake of clarity we reduced the complexity of the formulas by assuming that 
% $c^2 >s\log(s)$\fb{check}. 
$ c > \log(s) $. \bp{I think}
%
At inference time often some of the computations can be done only once (after training),
and then cached for every evaluation.
In the column \textit{Inference} the leading terms of 
% the cost only related to the evaluation stage 
these costs
can be found. Indeed, when it is possible (hence for every method except to SOC) we applied a \textbf{caching system} of the parameterized layers. This means that parameterization is performed only once and the result is stored in memory. A detailed explenation of these values can be found in the \Cref{sec:computational_complexity}.
% \input{tab/complexity}

\paragraph{Memory Requirements}
\bp{Actually, let's keep the table in I think.}
The amount of memory required for the training is an important factor.
It allows us to use bigger models or bigger batch sizes,
generally improving performance or decreasing training time.

% For an overview of training times see Table \ref{table:memory}.
% \input{tab/memory}

In general the memory required depends on two things:
the number of parameters of the model, and the number of activations
a model has.
% The number of parameters of a model is required for multiple reasons:

We need to store three floats for each parameter of the model.
We need to keep the parameters itself in memory in order to do the forward pass.
We also need to store each partial derivative in the backward pass.
Finally for our optimizer we also need to store the momentum term.

The number of values calculated in the forward pass is the other important term.
We generally need to keep those values in storage in order to propagate the
derivative back through a model.
Notably, this number depends on the batch size, and especially for small
models tends to be larger than the number of parameters.
For most method, the number of values calculated in the forward pass
is a sum of two values: We need to store some amount of floats for
the rescaling procedure, and some more to do the actual forward pass.
Since the rescaling procedure needs to be done only once per batch,
usually the forward pass is the more memory intensive part.
% This part is the same for most of the models.

\textbf{Measured:}
Usually applying transformations to the weights does require
less memory than storing the activations in the forward pass.
So in \cref{table:memory_from_transformations} 
we report for each method,
how much many transformations are done to the input in the 
forward pass, and how much much memory these require.
% Note that for example applying a convolution
% \input{tab/memory_from_transformations}


A notable exception is \Cayley.
This layer requires padding the weight to the size of the
input and calculating the fast Fourier transform of that.
This does require $\mathcal{O}(s^2 c^2)$,
potentially larger than the $b s^2 c$ memory required to
store each activation.


% We also show the memory required for the parameters
% as well as the transformations of the parameters,
% see \cref{table:memory_for_parameters}.
% \input{tab/memory_for_parameters}


For this part, \AOL, and \BnB require the same amount of memory as
a standard convolution. \CPL, \SLL and \SOC have an extra constant
factor more (2 for \CPL and \SLL, and for \SOC this is equal to the
number of iterations).
Other methods (\Cayley and \LOT and maybe \BCOP) require memory
scaling badly with the number of channels?
%\paragraph{Coverage Analysis (?)}
%Does the method parameterize all the 1-Lipschitz layers? Orthogonal only? etc etc..

\subsection{(Theoretical?) Observations}

\begin{comment}
\paragraph{Cayley:} The number of parameters for this method scales
like $s^2 c^2$. For high resolution inputs therefore in order to keep
the memory requirements reasonable we need to choose the number of
channels, $c$, fairly small. This then also means that the number
of floating point operations (which is $s^2 c^3$) is reasonable.
\prov{We conduct experiments with $c=16$.}


\paragraph{SOC:} Not that for this method, in the forward pass, 
the amount floats we need to store for each example is multiplied
by a factor of $t$, where $t$ is the number of inner iterations.
Since in the original paper $t=6$, and most of the memory is usually
used for saving the activations in the forward pass, 
% using SOC requires a lot more memory than compareable layers.
we do again need a fairly small $c$ in order to allow us to train the
network \fb{Discuss this point}.

\paragraph{BCOP}
Orthogonal Convolutions have shown to have at least $c^2$ connected components. To overcame this limitation the authors proposed to parameterize them with convolutions with a doubled number of channels in the same connected components. The cost of a BCOP is then almost the double of the cost of a single convolution but is independent on the input dimension.


\paragraph{\CPL:}
This layer requires a good estimation of the spectral norm of the weight matrix.
Assume that the estimation has a relative error of $\alpha < 1$.
(more precisely, the estimation of $\|W\|_2$ gives a value
smaller than $\alpha \|W\|_2$.)
Then, the Lipschitz constant of the layer might be up to
$1 + 2(1-\alpha)^2$ instead of $1$ we aimed for.
(realized for example if $W$ is the identity, $b$ the zero vector 
and all elements of $x$ are positive).

In our experiments, we found that using only 100 power iterations
to estimate $\|W\|_2$ causes the bound of the Lipschitz constant
of the whole network to be far from $1$ \fb{to discuss}.
In fact, we found it to be $7.2$ (made up value for now!),
showing that the robust accuracy reported by the original paper
might not be reliable.

We instead evaluated the model using $10.000$ power iterations,
and report the \cra evaluated in this way.
\end{comment}


==> tab/complexity.tex <==


\begin{table}[t]
% \setlength{\tabcolsep}{4pt}
\centering
\caption{
    Computational complexity in terms of FLOPS \fb{adjust} for
    batch size of $b$,
    image size (input and output) of $s \times s \times c$,
    $t$ inner iterations and kernel size $k \times k$.
    Denote by $C$ the complexity of the forward pass of a standard convolution. 
    ($C = c^2 k^2 s^2 b$ ). \\
}
\label{table:complexity}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|ll}

\hline \noalign{\smallskip}

Method & Training & Inference \\

\noalign{\smallskip} \hline \noalign{\smallskip}

Standard Convolution    & $C= c^2 k^2 s^2 b$    & $C$ \\
\powermeth  & $C + c^2 k^2 s^2$       & $C$   \\
% Fantastic4 & (\add{$4tc^2k^2 + C$})  & (\add{$C$})\\
%\BnB\footnotemark[1] & $tbc^2$ & $bc^2$ \\
\BCOP &$C+  ktc^3$& $C$\\
% \Cayley     & $s^2 c^3 + b c s^2 \log s$ \\
% Cayley:   - FFT on weights: c^2 s^2 log(s)
%           - FFT on inputs: b c s^2 log(s)
%           - inverting weights: s^2 c^3
%           - matrix-vector multiplication: b s^2 c^2
%\Cayley     & $s^2 c^3 + (b c + c^2) s^2 \log(s^2) + b s^2 c^2$    
%            & $b c s^2 \log(s^2) + b s^2 c^2$ \\
\Cayley     & $s^2 c^3 + b s^2 c^2$ & $b s^2 c^2$ \\
\SOC        & $C t_{\tt T} + 4\,c^2k^2$     & $C t_{\tt I}$   \\
\ECO        & $C  % dilated convolution
                +\frac{1}{2} k^2 c^3 t  % Orthogonalization
                % + c^2 k^2 \log(k)  % FFT
                $ & $C$\\
\AOL        & $C + c^3 k^4$      & $C$ \\
\LOT        & $t s^2 c^3 + bs^2c^2$ & $bs^2c^2$\\
% LOT:   - FFT on weights: c^2 s^2 log(s)
%           - FFT on inputs: b c s^2 log(s)
%           - inverse square root for every patch ts^2c^3
%           - matrix-vector multiplication: b s^2 c^2

\CPL        & $2C + c^2 k^2 s^2$      & $2C$ \\
\SLL        & $2C + c^3 k^4$      & $2C$ \\

\noalign{\smallskip} \hline \noalign{\smallskip}

\end{tabular}%
}
\end{table}


==> tab/complexity_OLD.tex <==


\begin{table}[t]
% \setlength{\tabcolsep}{4pt}
\begin{center}
\caption{
    \textbf{Convolutions.}
    Computational complexity for
    batch size $b$,
    image size $s \times s$,
    width (number of channels/units) $c$
    and $t$ number of inner iterations
    and kernel size $k \times k$.\\
    Denote by $C$ the complexity of the forward pass of a standard convolution. \\
    *2 denotes the complexity of calculating the spectral norm. \\
    \bp{Compare with throughput?}
}
\label{table:complexity}
\begin{tabular}{l|ll}

\hline \noalign{\smallskip}

Method & Complexity Training & Complexity Inference \\

\noalign{\smallskip} \hline \noalign{\smallskip}

Standard Convolution & $c^2 k^2 s^2 b$\add{$=:C$} & $c^2 k^2 s^2 b$ (\add{$C$}) \\
% \spec 
Standard Power method & $c^2$ (\add{$tc^2k^2 + C$})  & (\add{$C$})\\
Fantastic4 & (\add{$4tc^2k^2 + C$})  & (\add{$C$})\\

\BnB\footnotemark[1] & $c^2$ ?  (\add{$4t c^2b$}) & (\add{$c^2b$})\\  
\Cayley & $s^2 c^3 + b c s^2 \log s$ \\
SOC & $c^2 k^2 s^2 b t$ + normalization \\
ECO & \\
\AOL{} Convolution & $c^2 k^2 s^2 b + c^3 k^4$ & $c^2 k^2 s^2 b$ \\
\AOL{} Convolution & $ C * \left(1 + \frac{ck^2}{s^2b}\right)$ \\
\CPL & *2 & $C$ \\
\SLL & same as AOL & C \\

\noalign{\smallskip} \hline \noalign{\smallskip}

\end{tabular}
\end{center}
\footnotemark[1] Only applicable to linear layers ($k=1$)

% \setlength{\tabcolsep}{1.4pt}
\end{table}


==> tab/epochs_budget_1x1.tex <==


\begin{table}[h!]
\centering
\caption{Budget of training epochs for each model and different layers. Batch size and training time are set to be $256$ and $2$h respectively for all the architectures.}
  
\label{tab:budget}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|cc|cc|cc|cr}
\toprule
Model & $L_3$\hspace{1em} & $L_1$\hspace{1em} & $M_3$\hspace{1em} & $M_1$\hspace{1em} & $S_3$\hspace{1em} & $S_1$\hspace{1em} & $XS_3$\hspace{1em} & $XS_1$ \\
\midrule
AOL      &       83 &          125 &      367 &          648 &      763 &          972 &       837 &           961 \\
BCOP           &       24 &           37 &       94 &          137 &      125 &          165 &       127 &           167 \\
CPL      &      194 &          334 &      522 &          809 &      797 &          911 &       836 &           949 \\
Cayley     &       17 &           17 &       70 &           70 &      214 &          214 &       356 &           357 \\
LOT            &      - &          - &       11 &           15 &       68 &           87 &       222 &           234 \\
SLL      &       79 &          109 &      353 &          523 &      703 &          790 &       735 &           780 \\
SOC            &       77 &          133 &      201 &          310 &      336 &          384 &       371 &           410 \\
\midrule
Param.s (M) &     100.6 &         44.8 &     25.1 &         11.2 &      6.3 &          2.8 &       1.6 &           0.7 \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tab/greedy_search_CIFAR10.tex <==
\begin{table}[b]
\centering
\caption{Result of the greedy search performed for CIFAR10 on a span of $16$ random runs for each couple of method, model.
\bp{I think this table can be removed, all the results are reported in other tables as far as I know.}
}
\label{tab:main-comparison}

\begin{tabular}{ll|ccc|ccc}
\toprule
    & \textbf{Kernel Size} & \multicolumn{3}{c}{3 x 3} & \multicolumn{3}{c}{1 x 1} \\
    & {} & Rob.Acc [\%]\hspace{1em} & LR\hspace{1em} &    
    WD\hspace{1em} & Rob.Acc [\%]\hspace{1em} & LR\hspace{1em} &    WD \\
\textbf{Layer} & \textbf{Model} &         &       &       &         &       &       \\
\midrule
\textbf{AOL} & \textbf{L} &   48.18 &  2e-2 &  7e-5 &   45.12 &  3e-2 &  8e-5 \\
    & \textbf{M} &   54.96 &  2e-2 &  1e-4 &   50.42 &  2e-2 &  1e-4 \\
    & \textbf{S} &   55.32 &  1e-2 &  5e-5 &   49.56 &  5e-2 &  4e-5 \\
    & \textbf{XS} &   54.02 &  6e-2 &  4e-5 &   48.34 &  8e-2 &  7e-6 \\
\textbf{BCOP} & \textbf{L} &   44.78 &  1e-3 &  9e-6 &   44.48 &  4e-3 &  2e-4 \\
    & \textbf{M} &   53.42 &  6e-3 &  7e-6 &   48.96 &  8e-3 &  5e-6 \\
    & \textbf{S} &   53.54 &  4e-3 &  8e-5 &    48.9 &  4e-3 &  2e-5 \\
    & \textbf{XS} &   51.46 &  7e-3 &  3e-4 &   47.66 &  1e-2 &  7e-5 \\
\textbf{BnB} & \textbf{L} &       - &     - &     - &   48.34 &  3e-2 &  2e-4 \\
    & \textbf{M} &       - &     - &     - &    50.0 &  2e-2 &  4e-6 \\
    & \textbf{S} &       - &     - &     - &   49.62 &  2e-2 &  2e-5 \\
    & \textbf{XS} &       - &     - &     - &   47.18 &  8e-3 &  1e-4 \\
\textbf{CPL} & \textbf{L} &   55.04 &  5e-2 &  3e-4 &   48.36 &  8e-2 &  9e-6 \\
    & \textbf{M} &   58.92 &  8e-2 &  1e-4 &    54.1 &  1e-1 &  2e-4 \\
    & \textbf{S} &   57.52 &  7e-2 &  1e-4 &   54.52 &  9e-2 &  9e-5 \\
    & \textbf{XS} &   55.72 &  3e-2 &  1e-4 &    51.6 &  2e-2 &  1e-4 \\
\textbf{Cayley} & \textbf{L} &   39.48 &  8e-3 &  2e-4 &   36.88 &  2e-2 &  8e-5 \\
    & \textbf{M} &   52.34 &  1e-2 &  6e-6 &    42.9 &  2e-2 &  2e-5 \\
    & \textbf{S} &    56.0 &  1e-2 &  1e-5 &   47.28 &  1e-2 &  4e-6 \\
    & \textbf{XS} &   55.04 &  2e-2 &  2e-5 &   46.54 &  1e-2 &  2e-5 \\
\textbf{LOT} & \textbf{M} &   39.94 &  2e-2 &  9e-6 &   34.64 &  3e-2 &  7e-5 \\
    & \textbf{S} &    51.2 &  3e-2 &  7e-5 &   48.14 &  5e-2 &  3e-4 \\
    & \textbf{XS} &   55.26 &  8e-2 &  4e-6 &   45.76 &  2e-2 &  2e-4 \\
\textbf{SLL} & \textbf{L} &    32.5 &  6e-2 &  2e-4 &   45.42 &  9e-2 &  2e-4 \\
    & \textbf{M} &   53.28 &  9e-2 &  9e-5 &   53.88 &  7e-2 &  2e-4 \\
    & \textbf{S} &   55.96 &  4e-2 &  2e-4 &   53.32 &  3e-2 &  2e-4 \\
    & \textbf{XS} &   50.88 &  9e-2 &  2e-5 &   51.38 &  4e-2 &  1e-4 \\
\textbf{SOC} & \textbf{L} &   40.52 &  2e-2 &  2e-4 &   42.32 &  4e-2 &  9e-5 \\
    & \textbf{M} &   54.72 &  7e-2 &  1e-4 &   45.02 &  3e-2 &  7e-5 \\
    & \textbf{S} &    48.4 &  2e-2 &  2e-5 &    45.1 &  4e-2 &  6e-6 \\
    & \textbf{XS} &   49.98 &  5e-2 &  7e-6 &    44.1 &  7e-2 &  2e-5 \\
\bottomrule
\end{tabular}
\end{table}

==> tab/greedy_search_TinyImageNet.tex <==
\begin{table}[b]
\centering
\caption{Result of the greedy search performed for TinyImageNet on a span of $16$ random runs for each couple of method, model.}
\label{tab:main-comparison_TinyImageNet}
\begin{tabular}{ll|ccc}
\toprule
 &  & Rob.Acc & LR & WD \\
Layer & Model &  &  &  \\
\midrule
\multirow[t]{4}{*}{\textbf{AOL}} & \textbf{TL} & 9.0 & 2e-2 & 8e-6 \\
\textbf{} & \textbf{TM} & 13.5 & 4e-2 & 8e-6 \\
\textbf{} & \textbf{TS} & 13.5 & 7e-2 & 5e-6 \\
\textbf{} & \textbf{TXS} & 12.0 & 3e-2 & 2e-5 \\
\cline{1-5}
\multirow[t]{4}{*}{\textbf{BCOP}} & \textbf{TL} & 1.7 & 1e-4 & 3e-4 \\
\textbf{} & \textbf{TM} & 7.6 & 3e-4 & 1e-4 \\
\textbf{} & \textbf{TS} & 6.9 & 7e-4 & 4e-5 \\
\textbf{} & \textbf{TXS} & 4.7 & 6e-4 & 5e-5 \\
\cline{1-5}
\multirow[t]{4}{*}{\textbf{CPL}} & \textbf{TL} & 10.4 & 6e-2 & 1e-5 \\
\textbf{} & \textbf{TM} & 12.9 & 4e-2 & 2e-5 \\
\textbf{} & \textbf{TS} & 12.5 & 4e-2 & 3e-5 \\
\textbf{} & \textbf{TXS} & 12.6 & 1e-1 & 9e-6 \\
\cline{1-5}
\multirow[t]{4}{*}{\textbf{Cayley}} & \textbf{TL} & 0.6 & 1e-3 & 3e-4 \\
\textbf{} & \textbf{TM} & 6.9 & 4e-3 & 4e-5 \\
\textbf{} & \textbf{TS} & 11.3 & 5e-3 & 7e-5 \\
\textbf{} & \textbf{TXS} & 11.7 & 8e-3 & 8e-5 \\
\cline{1-5}
\multirow[t]{3}{*}{\textbf{LOT}} & \textbf{TM} & 3.0 & 2e-2 & 6e-6 \\
\textbf{} & \textbf{TS} & 12.0 & 5e-2 & 1e-4 \\
\textbf{} & \textbf{TXS} & 14.2 & 3e-2 & 2e-4 \\
\cline{1-5}
\multirow[t]{4}{*}{\textbf{SLL}} & \textbf{TL} & 1.8 & 7e-2 & 1e-4 \\
\textbf{} & \textbf{TM} & 4.9 & 5e-2 & 5e-5 \\
\textbf{} & \textbf{TS} & 10.6 & 4e-2 & 2e-4 \\
\textbf{} & \textbf{TXS} & 11.8 & 7e-2 & 3e-4 \\
\cline{1-5}
\multirow[t]{4}{*}{\textbf{SOC}} & \textbf{TL} & 6.9 & 6e-2 & 1e-4 \\
\textbf{} & \textbf{TM} & 11.4 & 7e-2 & 1e-4 \\
\textbf{} & \textbf{TS} & 9.0 & 7e-2 & 2e-5 \\
\textbf{} & \textbf{TXS} & 11.2 & 9e-2 & 1e-4 \\
\cline{1-5}
\bottomrule
\end{tabular}

\end{table}

==> tab/memory.tex <==


\begin{table}[t]
% \setlength{\tabcolsep}{4pt}
\begin{center}
\caption{
    \textbf{Memory Requirements.}
    Computational complexity for
    batch size $b$,
    image size $s \times s$,
    width (number of channels/units) $c$
    and $t$ number of inner iterations
    and kernel size $k \times k$.\\
    We will give values in terms of order of magnitude $\mathcal{O}$,
    and maybe assume matrix multiplication requires memory of $\mathcal{O}(n^2)$? \\
    We will (maybe) assume $b \ge k^2$ to simplify the terms. \fb{This table has to be removed?}
}
\label{table:memory}
\begin{tabular}{l|llll|llll}

\hline \noalign{\smallskip}

% Method & Number of Parameters & Floats Forward Pass \\
Method & \multicolumn{4}{c|}{Parameters} & \multicolumn{4}{c}{Memory} \\

\noalign{\smallskip} \hline \noalign{\smallskip}

\stdconv        & $c^2$ & $k^2$ &&     & $b$ & $s^2$ & $ c$     \\
\powermeth      & $c^2$ & $k^2$ &&     & $b$ & $s^2$ & $ c$     \\
\BCOP \\
\Cayley         & $c^2$ & & $s^2$ &    & \\
\SOC            & $c^2$ & $k^2$ &&     & $b$ & $s^2$ & $ c$ & $ t$     \\
\AOL            & $c^2$ & $k^2$ &&     & $b$ & $s^2$ & $ c$     \\
\LOT \\
\CPL \\
\SLL \\

\noalign{\smallskip} \hline \noalign{\smallskip}
\end{tabular}
\end{center}

% \setlength{\tabcolsep}{1.4pt}
\end{table}


==> tab/memory_for_parameters.tex <==


\newcommand{\NONE}{-}

\begin{table}[t]
% \setlength{\tabcolsep}{4pt}
\begin{center}
\caption{
    \textbf{Memory Requirements.}
    Memory requirements to store parameters
    as well as do transformations of those parameters.
    We consider batch size $b$,
    image size $s \times s \times c$,
    $t$ number of inner iterations
    and kernel size $k \times k$.\\
    %
    We compare the memory requirements to the one of 
    a standard convolution, $k^2 s^2$, the size of the kernel.
    %
    \warning{Also double and triple check here}
}
\label{table:memory_for_parameters}
\begin{tabular}{l|l|l}

\hline \noalign{\smallskip}

% Method & Number of Parameters & Floats Forward Pass \\
Method  & Parameter         & Memory \\
        & Transformation    &  \\

\noalign{\smallskip} \hline \noalign{\smallskip}

\stdconv & \NONE                & $C = k^2 c^2$ \\
\powermeth & \NONE              & $C + s^2 c$ \\
\BCOP   & \CONV                 & $C + \mathcal{O}(k^4 c^2)$ \\
\Cayley & $2\times$ \FFT \& \MV & $3 C + s^2 c^2$ \\
\SOC    & $t\times$ \CONV       & $t C$     \\
\AOL    & \CONV                 & $C + \mathcal{O}(k^2 c^2)$ \\
\LOT    &                       & \\
\CPL    & $2\times$ \CONV + \ACT & $2C + s^2ct$ \\
\SLL    & $2\times$ \CONV + \ACT & $2C + \mathcal{O}(k^2 c^2)$\\

\noalign{\smallskip} \hline \noalign{\smallskip}
\end{tabular}
\end{center}

% \setlength{\tabcolsep}{1.4pt}
\end{table}




==> tab/memory_from_transformations.tex <==

% \newcommand{\CONV}{CONV}
% \newcommand{\FFT}{FFT}
% \newcommand{\MATMUL}{MATMUL}
% \newcommand{\MV}{MV}  % Matrix-vector product
% \newcommand{\ACT}{ACT}  % (..ivation)



\begin{table}[t]
% \setlength{\tabcolsep}{4pt}
\begin{center}
\caption{
    \textbf{Memory Requirements.}
    Computational complexity for
    batch size $b$,
    image size $s \times s$,
    width (number of channels/units) $c$
    and $t$ number of inner iterations
    and kernel size $k \times k$.\\
    %
    Each transformation requires an additional
    memory equal to the input size,
    $C = b s^2 c$.
    %
    We assume adding a bias and applying an activation
    after doing a convolution does not require any
    additional memory.
    The transformations we report are
    convolutions (\CONV),
    fast fourier transformations (\FFT),
    matrix-vector multiplications (\MV),
    as well as applications of an activation function (\ACT).
    %
    Note that all layers (apart from \BCOP) require an
    additional $k^2 c^2$ float memory in order to store
    the weights.
    \warning{Also double and triple check here}
}
\label{table:memory_from_transformations}
\begin{tabular}{l|l|l}

\hline \noalign{\smallskip}

% Method & Number of Parameters & Floats Forward Pass \\
Method & Transformation & Memory \\

\noalign{\smallskip} \hline \noalign{\smallskip}

\stdconv & \CONV                & $C$ \\
\powermeth & \CONV              & $C + s^2 c$ \\
\BCOP   & \CONV                 & $C + \mathcal{O}(k^3 c^2)$ \\
\Cayley & $2\times$ \FFT + \MV  & $3 C + s^2 c^2$ \\
\SOC    & $t\times$ \CONV       & $t C$     \\
\ECO    & \CONV                 & $C + \mathcal{O}(k^2 c^2 t)$ \\
\AOL    & \CONV                 & $C + \mathcal{O}(k^2 c^2)$ \\
\LOT    & $2\times$ \FFT + \MV  & $3 C + \mathcal{O}(s^2 c^2 t)$ \\
\CPL    & $2\times$ \CONV + \ACT & $2C + s^2c$ \\
\SLL    & $2\times$ \CONV + \ACT & $2C + \mathcal{O}(k^2 c^2)$\\

\noalign{\smallskip} \hline \noalign{\smallskip}
\end{tabular}
\end{center}

% \setlength{\tabcolsep}{1.4pt}
\end{table}




==> tab/sizes.tex <==




\setlength{\tabcolsep}{4pt}
\begin{table}[t]
\begin{center}
\caption{
    Allowed number of parameters for different models,
    as well as the width parameter such that
    the architecture in \cref{table:architecture}
    is of corresponding size.
}
\label{table:sizes}

\begin{tabular}{lll}
\noalign{\smallskip} \hline \noalign{\smallskip}
Size & Parameters (millions) & Width parameter \\
%         & Parameters    & Width     \\
% Size    & (millions)    & parameter \\
\noalign{\smallskip} \hline \noalign{\smallskip}

XS  & $<2$      & $16$  \\
S   & $<8$      & $32$  \\
M   & $<32$     & $64$  \\
L   & $<128$    & $128$   \\

\noalign{\smallskip} \hline

\end{tabular}

% \begin{tabular}{llc}
% \noalign{\smallskip} \hline \noalign{\smallskip}
% Size & $w$ &  Parameters (millions)\\
% \noalign{\smallskip} \hline \noalign{\smallskip}
% XS  & $16$  & $1 < p < 2$ \\
% S   & $32$  & $4 < p < 8$ \\
% M   & $64$  & $16 < p < 32$ \\
% L   & $128$ & $\ \ 64 < p < 128$  \\
% \noalign{\smallskip} \hline
% \end{tabular}


\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}







==> tab/theoretical_both.tex <==



% \newcommand{\CONV}{CONV}
% \newcommand{\FFT}{FFT}
% \newcommand{\MATMUL}{MATMUL}
% \newcommand{\MV}{MV}  % Matrix-vector product
% \newcommand{\ACT}{ACT}  % (..ivation)



\begin{table*}[t]
% \setlength{\tabcolsep}{4pt}
\begin{center}
\caption{
    % \textbf{Memory Requirements.}
    \textbf{Computational complexity and memory requirements of different layers.}
    % Computational complexity for
    % batch size $b$,
    % image size $s \times s \times c$,
    % $t_{\texttt{T}}$ and $t_{\texttt{I}}$ inner iterations (at training and at inference)
    % and kernel size $k \times k$.\\
    % %
    We show the (most costly) transformations applied to the input as well
    as to the weights for different layers.
    We also show the multiply-accumulate operations (MACS)
    needed during training as well as during inference.
    Finally, we also show the memory requirements (per layer) 
    % for doing backpropagation. \\
    for training the model. \\
    %
    For a detailed explanation on what is reported see \cref{sec:table_explanation}.
    For some reasoning how those values were
    derived see \cref{sec:computational_complexity}.
    %
    % We use $C$ to denote the MACS of a convolution, 
    % $C= c^2 k^2 s^2 b$ the complexity of a convolution.
    % % 
    % Each transformation requires an additional
    % memory equal to the input size,
    % $M = b s^2 c$.
    % Furthermore, we define $P$ as the size of the
    % kernel of a standard convolution, $P = c^2 k^2$.
    % %
    % We assume adding a bias and applying an activation
    % after doing a convolution does not require any
    % additional memory.
    % We also assume that rescaling with a constant
    % value does not require additional memory. \bp{?}
    % The transformations we report are
    % convolutions (\CONV),
    % block convolutions (\BCONV),
    % fast Fourier transformations (\FFT),
    % matrix-vector multiplications (\MV),
    % matrix inversion (\INV),
    % normalization (\NORM),
    % (one step of) power iteration (\PM),
    % as well as applications of an activation function (\ACT).
    % %
    % Note that all layers (apart from \BCOP) require an
    % additional $k^2 c^2$ float memory in order to store
    % the weights.
    % \bp{Use MACS, FLOPS or O()?}
    \warning{Also double and triple check here}
    % \bp{Look at code in order to validate coefficient 
    % e.g. for Cayley.}
    % \bp{To discuss: Do we use order notation or not.
    % E.g. matrix multiplication is $2c^3$ flops afaik,
    % not even sure about convolutions.
    % Maybe we could use MAC (= Multiply–accumulate operation) instead?\fb{?}}
}
\label{table:theoretical}
\begin{tabular}{l|ll|ll|l}

\hline \noalign{\smallskip}

% Method & Number of Parameters & Floats Forward Pass \\
Method  & Input             & Parameter            & Training  & Inference     & Training \\
%         & Transformation    & Transformations   & FLOPS     & FLOPS      & Memory  \\
        & Transformation    & Transformations   & MACS $\OO(\cdot)$      & MACS ($\OO$)         & Memory\footnotemark[2]  \\

\noalign{\smallskip} \hline \noalign{\smallskip}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Order of variables: b s c k t %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\stdconv & \CONV & - & $C$ & $C$ & $M + P$ \\
\BCOP & 
\CONV & $2k\times$ BnB + $k^3\times$ \MATMUL & % $k^2/2 \times$ \ORTH + $2k \times$ \BCONV & 
% $C+  \mathcal{O}(ktc^3) + \mathcal{O}(k^3 c^3)$ 
%         & $C$ & $M + \mathcal{O}(k t c^2) + \mathcal{O}(k^3 c^2)$ \\
% $C+  \mathcal{O}(k(t+k^2)c^3)$ & $C$ & $M + \mathcal{O}(k (t+k^2) c^2)$ \\
$C+  \mathcal{O}(c^3 k (k^2 + \tTrain))$ & $C$ & $M + \mathcal{O}(c^2 k (k^2 + \tTrain))$ \\
% BCOP:     - Orthogonalization: O(ktc^3) MACS & O(ktc^2) memory
%           - Kernel assembly:   O(k^3 c^3) MACS & O(k^3 c^2) memory

\Cayley & 
% Cayley:   - FFT on weights: c^2 s^2 log(s)
%           - FFT on inputs: b c s^2 log(s)
%           - inverting weights: s^2 c^3
%           - matrix-vector multiplication: b s^2 c^2
% $2\times$ \FFT + $2\times$ \MV & $c^2 \times$ \FFT + $s^2\times$ \INV & 
$2\times$ \FFT + $\frac{1}{2}s^2\times$ \MV & $c^2 \times$ \FFT + $s^2\times$ \INV & 
% $b s^2 c^2 + s^2 c^3$ & $b s^2 c^2$ & $4M + \mathcal{O}(P)$ \\
$\frac{1}{2} b s^2 c^2 + s^2 c^3$ & $\frac{1}{2} b s^2 c^2$ & $4M + \mathcal{O}(s^2 c^2)$ \\

% \Cayley(2) & 
% % Cayley:   - FFT on weights: c^2 s^2 log(s)
% %           - FFT on inputs: b c s^2 log(s)
% %           - inverting weights: s^2 c^3
% %           - matrix-vector multiplication: b s^2 c^2
% $2\times$ \FFT + $2\times$ \MV & \FFT + $s^2\times$ \INV & 
% % $b s^2 c^2 + s^2 c^3$ & $b s^2 c^2$ & $4M + \mathcal{O}(P)$ \\
% $b s^2 c^2 + s^2 c^3$ & $b s^2 c^2$ & $4M + \mathcal{O}(s^2 c^2)$ \\


\SOC    & 
$t\times$ \CONV & F4 & 
% $C t_{\texttt{T}}$ & $C t_{\texttt{I}}$ & $M t_{\texttt{T}} + P$     \\
$C \tTrain$ & $C \tTest $ & $M \tTrain + P$     \\

% \ECO    &
% \CONV & $k^2 t/2 \times$ \MATMUL + $c^2 \times$ \FFT & % dilated convolution + orthogonalization
% $C +\frac{1}{2} k^2 c^3 t$ & $C$ & $M + \mathcal{O}(k^2 c^2 t)$ \\
                
\AOL    & 
\CONV  & $c \times$ \CONV & %SELF-CONV & 
$C + \Ord{c^3 k^4}$      & $C$ & $M + \mathcal{O}(P)$ \\

\LOT    & 
$2\times$ \FFT + \MV  & $c^2 \times$ \FFT + $4 s^2 t \times$ \MATMUL &
$b s^2c^2 + 4s^2 c^3 t$ & $b s^2c^2$ & $3M + \mathcal{O}(s^2 c^2 \tTrain)$ \\

\CPL    & 
$2\times$ \CONV + \ACT & \CONV & % \PM & 
$2C$      & $2C$ & $3M + P$ \\

\SLL    & 
$2\times$ \CONV + \ACT & $c \times$ \CONV & %SELF-CONV &
$2C + \Ord{c^3 k^4}$ & $2C$ & $3M + \mathcal{O}(P)$ \\

\noalign{\smallskip} \hline \noalign{\smallskip}
\end{tabular}
\footnotetext[2]{\fb{To be properly defined}}

\end{center}


% \setlength{\tabcolsep}{1.4pt}
\end{table*}




==> tab/training_times.tex <==


\setlength{\tabcolsep}{4pt}
\begin{table}[t]
\begin{center}
\caption{
    \textbf{Training time} in minutes per epoch on \CIFARS
    for different layer types and model size.
    \bp{I'll put this table to the appendix after finishing writing
        section 5.1.}
}
\label{table:training_times}

\begin{tabular}{l|llll}
\noalign{\smallskip} \hline \noalign{\smallskip}
 & \multicolumn{4}{c}{Model size} \\

 & XS & S & M & L \\ 
\noalign{\smallskip} \hline \noalign{\smallskip} 
AOL & 0.15 & 0.17 & 0.33 & 1.43 \\ 
BCOP & 0.94 & 0.93 & 1.27 & 4.99 \\ 
CPL & 0.15 & 0.16 & 0.24 & 0.63 \\ 
Cayley & 0.32 & 0.58 & 1.82 & 6.97 \\ 
LOT & 0.52 & 1.75 & 10.24 & - \\ 
SLL & 0.16 & 0.16 & 0.33 & 1.52 \\ 
SOC & 0.33 & 0.36 & 0.59 & 1.56 \\ 
Standard & 0.10 & 0.11 & 0.20 & 0.51 \\



\noalign{\smallskip} \hline
\end{tabular}

\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}



